Efficient Quantum Algorithms for (Gapped) Group Testing and Junta Testing

In the $k$-junta testing problem, a tester has to efficiently decide whether a given function $f:\{0,1\}^n\rightarrow \{0,1\}$ is a $k$-junta (i.e., depends on at most $k$ of its input bits) or is $\epsilon$-far from any $k$-junta. Our main result is a quantum algorithm for this problem with query complexity $\tilde O(\sqrt{k/\epsilon})$ and time complexity $\tilde O(n\sqrt{k/\epsilon})$. This quadratically improves over the query complexity of the previous best quantum junta tester, due to At\i c\i\ and Servedio. Our tester is based on a new quantum algorithm for a gapped version of the combinatorial group testing problem, with an up to quartic improvement over the query complexity of the best classical algorithm. For our upper bound on the time complexity we give a near-linear time implementation of a shallow variant of the quantum Fourier transform over the symmetric group, similar to the Schur-Weyl transform. We also prove a lower bound of $\Omega(k^{1/3})$ queries for junta-testing (for constant $\epsilon$).

==> other.tex <==
In this section we give several other quantum testing results.



\subsection{The \atici-Servedio algorithm}
\label{sec:fouriersample}

We start by including for completeness the elegant quantum junta tester of \atici and Servedio~\cite{atici:testingJuntas}.
Their algorithm repeatedly uses Fourier sampling, which is the quantum procedure due to Bernstein and Vazirani~\cite{bernstein:quantumComplexity} described in \rf(alg:fourierSampling). It is straightforward to check its correctness, as the state of the algorithm before the measurement is $\sum_{S\subseteq [n]} \hf(S)\ket|S>$.


\begin{algorithm}[htb]
\algcaption{Fourier Sampling Subroutine\\
Input:& oracle access to a function $f\colon \cube\to\sbool$.\\
Output:& a subset $S\subseteq[n]$ returned with probability $\hf(S)^2$.}
\label{alg:fourierSampling}
\enumstart
\item Start with $n$-qubit state $\ket|0>$ and apply Hadamard gates to each qubit to form the uniform superposition $\frac{1}{\sqrt{2^n}}\sum_{x\in\01^n}\ket|x>$.
\item Apply a phase-query to $f$ to obtain $\frac{1}{\sqrt{2^n}}\sum_{x\in\01^n}f(x)\ket|x>$.
\item Apply Hadamard transforms to each qubit and measure.
\enumend
\end{algorithm}

The \atici-Servedio algorithm is a \emph{non-adaptive} quantum junta tester.
It applies Fourier sampling $O(k/\eps)$ times and takes the union of all the returned subsets.  The tester accepts iff the size of the union does not exceed $k$. 

Obviously, the algorithm always accept a $k$-junta.  
Assume now that the samples in the \atici-Servedio algorithm are made one by one. If $f$ is $\eps$-far from any $k$-junta and the union~$W$ of the sets seen so far has size at most~$k$, then by Lemma~\ref{lem:weightonextravars}, with probability at least~$\eps$ the next Fourier sample produces a subset $S$ not fully contained in~$W$, in which case $W$ grows.  Hence after an expected number of $O(k/\eps)$ samples, the set $W$ contains more than $k$ elements and we can reject~$f$ with certainty.

As noted in~\cite{montanaro:quantumProperyTest}, it is possible to improve the complexity of the algorithm to $O(k/\sqrt{\eps})$ at the cost of making it adaptive.  For that, keep track of the union~$W$ of the sampled subsets, and, if its size does not exceed $k$, try to extend $W$ using \rf(alg:testInfluence) with $\delta=\eps$. If $f$ is $\eps$-far from any $k$-junta, then an expected number of $O(k)$ runs of \rf(alg:testInfluence) will find more than $k$ relevant variables. (A similar improvement was also used in~\cite{chakraborty:quantumTestLinearity}.)

\begin{algorithm}
\algcaption{Test Influence of a Subset\\
Input:& a subset $V\subseteq[n]$, real $0<\delta<1$, and oracle access to $f\colon \cube\to\sbool$.\\
Assumption:& $\Inf_V(f)\ge\delta$.\\
Output:& a subset $S$ satisfying $\hf(S)\ne 0$ and $S\cap V\ne\emptyset$.}
\label{alg:testInfluence}
\enumstart
\item Perform $O(\sqrt{1/\delta})$ rounds of amplitude amplification on the Fourier sampling procedure, amplifying the subsets $S$ that intersect with $V$.
\item Measure a subset $S$.
\enumend
\end{algorithm}


\subsection{Fourier dimensionality}

Here we observe that the \atici-Servedio algorithm (\rf(sec:fouriersample)) is quite general and can be applied to other problems than junta testing as well. For example, Gopalan \etal study the problem of testing \emph{Fourier dimensionality}~\cite{gopalan:FourierDimensionality}. A function $f$ has Fourier dimensionality $k$ iff its spectrum is contained in a $k$-dimensional subspace of $\bF_2^n$, or (alternatively but equivalently) iff it can be represented as a function of $k$ characters $\chi_{s_1},\dots,\chi_{s_k}$.

Gopalan \etal constructed a non-adaptive randomized algorithm that $\eps$-tests Fourier $k$-di\-men\-sio\-na\-li\-ty in $O(k2^{2k}/\eps)$ queries, and proved a lower bound of $\Omega(2^{k/2})$ for the same task, even for adaptive algorithms. On the other hand, similarly to \rf(lem:weightonextravars), if $W$ is a $k$-dimensional subspace of $\bF_2^n$, and $f$ is $\eps$-far from any Fourier $k$-dimensional function, then $\sum_{S\colon S\notin W} \hf(S)^2\ge\eps$.  This means that the \atici-Servedio algorithm can be applied in this setting as well: instead of keeping track of the \emph{union} of the sampled Fourier coefficients, we keep track of their \emph{span} in $\bF_2^n$.  This gives the following result, exponentially improving over the best classical complexity:

\begin{thm}
The quantum query complexity of $\eps$-testing Fourier $k$-dimensionality is $O(k/\eps)$ for non-adaptive, and $O(k/\sqrt{\eps})$ for adaptive algorithms.
\end{thm}




\subsection{Support size}
\label{sec:supprotSize}

\onote{5/20: Alexander suggests to remove this section}


In this section we observe that the \qggt algorithm from \rf(sec:groupTesting), 
when viewed properly, can be used to solve the problem of 
testing the support size of a distribution.  

In the original definition of the distribution testing 
model~\cite{bravyi:testingDistributions,chakraborty:testingDistributions},
a probability distribution on $[n]$ is provided to the algorithm
through an oracle $O_f$ for a function $f\colon[m]\to[n]$
with the property that $|f^{-1}(i)|/m$ is the probability of an element $i \in [n]$.
\onote{5/19: moved here:}
This naturally leads to the following quantization of testing support size of a distribution.


Here we consider a more general model in which we are given an oracle
$O_\psi$ that outputs a pure quantum state ${\psi}$, a measurement of which 
in the standard basis yields the distribution on $[n]$.
We do this both because we find this model more natural in the quantum setting, and because
our results (as well as those 
in~\cite{bravyi:testingDistributions,chakraborty:testingDistributions})
naturally extend to it.
Notice that given the oracle $O_f$, one can prepare a state $\psi$ by running $O_f$ on the uniform superposition over the domain $[m]$. On the other hand, given access to $O_\psi$, it is hard to simulate $O_f$.

In more detail, let $\reg A$ be an $n$-dimensional quantum register, and $\reg W$ be an arbitrary quantum register. For $S\subseteq [n]$, let $\Pi_S$ be a projector in $\reg A$ that projects on the subspace spanned by the basis elements $\{\ket A|i>\mid i\in S\}$.  
We are given an oracle $O_\psi$ that maps $\ket AW|0>$ to some quantum state $\ket AW|\psi>$.
We are promised that $\psi$ satisfies one of the following two conditions:
\itemstart
\item $\psi$ is \emph{$k$-supported}, that is, there exists a $k$-subset $S\subseteq[n]$ such that $(\Pi_S\otimes I)\psi = \psi$; or
\item $\psi$ is $\eps$-far from any $k$-supported state, i.e., for any $k$-subset $S\subseteq[n]$, we have $\|(\Pi_S\otimes I)\psi\|^2\le 1-\eps$.
\itemend
We view this problem as a quantum counterpart of the problem of testing the support size of a probability distribution.

\begin{thm}
\label{thm:supportTester}
There exists a bounded-error quantum algorithm that distinguishes $k$-supported states from states that are $\eps$-far from any $k$-supported state, in
\(
O\sA[\sqrt{k/\eps}\log k]
\)
quantum queries. 
\end{thm}

\pfstart
We can use the same \rf(alg:juntaTester) to solve this problem.  The only difference is that instead of the Influence Tester of \rf(lem:infTester), we use the following procedure.  Given a subset $V\subseteq[n]$, and a real $\delta>0$, we perform $O(\sqrt{1/\delta})$ rounds of amplitude amplification on the input oracle $O_\psi$, amplifying the basis states in $V$. Thus, we are able to distinguish the case $\Pi_V\psi =0$ from the case $\|\Pi_V\psi\|^2\ge\delta$.\onote{5/18: was $\eps$}

Other than that, the analysis in \rf(sec:qalgs) goes through in this case, if we replace $\Inf_S(f)$ with $\|\Pi_S\psi\|^2$.  In the proof of \rf(lem:B0case), we can replace $\SubInf_S(f)$ with the same expression $\|\Pi_S\psi\|^2$, as it is linear in $S$.
\pfend

\onote{5/19: added:}
As remarked earlier, any tester in our model immediately implies a tester in the
original model~\cite{bravyi:testingDistributions,chakraborty:testingDistributions}:

\begin{cor}
\label{cor:rangeSize}
The image size can be tested in \(O\sA[\sqrt{k/\eps}\log k]\) quantum queries.
\end{cor}

\pfstart
Apply \rf(thm:supportTester) to the oracle $O_\psi$ that prepares the state 
\[
\psi = \frac1{\sqrt{m}} \sum_{x\in [m]} \ket A|f(x)> \ket W|x>. \qedhere
\]
\pfend

In the next section, we show that the problem of testing the image size can be also reduced to junta testing (in somewhat restricted settings).

However, the application scope of \rf(thm:supportTester) is broader than that of \rf(cor:rangeSize). The following corollary provides a simple example.

%We say that a function $f\colon\cube\to\bR$ is \emph{$k$-sparse} if it has at most $k$ non-zero Fourier coefficients.

\begin{cor}
\label{cor:fourierSparse}
There exists a bounded-error $O\sA[\sqrt{k/\eps}\log k]$-query
quantum algorithm that, given oracle access to a function $f\colon \{0,1\}^d \to\{\pm1\}$, distinguishes whether 
\itemstart
\item $f$ has at most $k$ non-zero Fourier coefficients, or
\item for any collection $\cS$ of $k$ subsets of $[d]$, we have $\sum_{T\in\cS} \hf(T)^2 \le 1-\eps$.
\itemend
\end{cor}

Note that this problem is \emph{not} a testing problem in the usual sense, because if a function $f$ does not fall in the second class, it does not mean that it is $\eps$-close to a function in the first class.
However, this problem is related to the corresponding testing problem, see~\cite{gopalan:FourierDimensionality} for more detail.

\pfstart[Proof of \rf(cor:fourierSparse)]
%Given the complexity we are aiming at, we may assume that $\eps\le 1/(5k)$.  By~\cite[Theorem 6]{gopalan:FourierDimensionality}, if $f$ is $\sqrt{\eps}$-close to a $k$-sparse \emph{real} function in $\ell_2$-norm, then it is $\eps/2$-close to a $k$-sparse \emph{Boolean} function. 
Apply \rf(thm:supportTester) with $n=2^d$ to the oracle $O_\psi$ that prepares the state
\[
\psi = \sum_{S\subseteq[n]} \hf(S) \ket A|S>
\]
using the subroutine in \rf(alg:fourierSampling).
\pfend

%Although, as we think, the query complexity of the algorithm in \rf(thm:supportTester) is close to optimal, its \emph{running time} is linear in $n$ that may seem not satisfactory.  Because of that, in \rf(sec:alternativeSupport), we give an alternative algorithm that has worse dependence on $\eps$, slightly worse on $k$, but has running time only polylogarithmic in $n$.  This algorithm is based on techniques from~\cite{bravyi:testingDistributions}.

==> sparsity.tex <==
\bnote{Major revision: restate as support size tester, emphasise time complexity...}

Recall the problem of testing the support size of a quantum state from \rf(sec:supprotSize).  
We are given an oracle $O_\psi$ that maps $\ket AW|0>$ to some quantum state $\ket AW|\psi>$.
We are promised that $\psi$ is either $k$-supported, or is $\eps$-far from any such state.
We have to distinguish the two cases.
Throughout this section, for $a\in[n]$, we use $p_a$ to denote the probability $\|\Pi_{\{a\}}\psi\|^2$.
\onote{11/17: we should define the testing support size problem in a ``definition'' environment, now that it plays such an important role in the paper. This would save us the repetition.}

In \rf(thm:supportTester), we gave a quantum algorithm with query complexity $O(\sqrt{k/\eps}\log k)$.
Unfortunately, the time complexity of the algorithm is linear in $n$, the dimension of the register $\reg A$.
In this section, we give a different algorithm for this problem using techniques from~\cite{bravyi:testingDistributions}.  The algorithm has slightly worse query complexity, but only logarithmic dependence of the running time on $n$.

\bnote{$s\gets c/k$}

\begin{algorithm}[htb]
\algcaption{Alternative Quantum Tester of Support Size\\
Input:& {Integer $k>0$, real $0<\eps<1$, and oracle $O_\psi$.}\\
Output:& Accepts if $\psi$ is $k$-supported; rejects if $f$ is $\eps$-far from being $k$-supportive.
}
\label{alg:kSparse}
\enumstart
\item
Let $\gamma$ be such that $(1+\gamma)^3=(1+\eps/5)$.
\item
Run \rf(sbrtn:estimateNW) with parameters $s=\eps/(4k)$ and $\gamma$, obtain an estimate $W$.
\item 
Run \rf(sbrtn:estimateNW) with parameters 
$s= \sA[(1-\gamma)\eps]/\sA[4(1+\gamma)k]$ and $\gamma$,
obtain an estimate $N$.
\item
Accept iff $W\geq 1-\eps/3$ and $N\leq (1+\eps/4)k$.
\enumend

\sbrtncaption{Count Large Fourier Coefficients\\
Input:& real numbers $s$, $\gamma$.\\
Output:& an estimate $N$ for the number of $a\in[n]$ satisfying $p_a \geq s$, and an estimate $W$ for the sum of such $p_a$'s.}
\label{sbrtn:estimateNW}
\enumstart
\item
Define recursively $s_0=s$ and $s_{i+1}= (1+\gamma) s_i$.
Let $\ell$ be the smallest number for which $s_\ell\ge1$.
\item
For each $i\in\{0, 1, \ldots, \ell-1\}$,
use amplitude estimation to get an estimate $q_i$ for the acceptance probability of the following subroutine with multiplicative precision $1\pm\gamma$ and correctness probability
$\ge 1-1/3\ell$.
\negmedskip
\itemstart
\item
Measure $\psi$ in the computational basis, and get an element $a\in[n]$ with probability $p_a$.
\item 
Use amplitude estimation to obtain an estimate $r$ to $p_a$ such that 
$|r-p_a|\leq \gamma p_a/3$.  Require correctness probability $\ge 1-\delta$, where $\delta=s^2$
\item 
Accept iff $r\in [s_i, s_{i+1}]$.
\itemend
\item
Output $W=\sum_i q_i$, $N=\sum_i q_i/s_i$. 
\enumend

\end{algorithm}

\onote{is it obvious how to get such approximation? it seems impossible if $\widehat{f}(S)$ is tiny, no? and how can we guarantee such an error if we don't know $\widehat{f}(S)$?}

%If the precision for the estimation step is sufficiently good, the probability that this algorithm outputs 1 is a good approximation to the sum of all $|\widehat{f}(S)|^2\in [p_0, p_1]$. \onote{do you mean $p,q$?}

\begin{thm}
\rf(alg:kSparse) distinguishes $k$-supported states from states that are $\eps$-far from any $k$-supported state, in
\( O\s[(\sqrt{k} \log^2 k \log \log k)/\eps^2] \)
quantum queries.  The algorithm has time complexity $\tO\s[(\sqrt{k}\log n)/\eps^2]$.
\end{thm}

\pfstart
Correctness of the algorithm follows from the following lemma.

\begin{lem}
\label{lem:estCorrect}
Fix $s$.  Let $\delta=s^2$, $N_s$ denote the true number of $a$ satisfying $p_a^2 \geq s$, and $W_s$ denote the sum of $p_a$ over all such $a$.
With probability at least 2/3, the estimates returned by \rf(sbrtn:estimateNW) satisfy
\begin{gather*} 
(1-\gamma)(1-\delta) W_{s/(1-\gamma)} \leq W 
\leq (1+\gamma) W_{s/(1+\gamma)} + (1+\gamma) \delta \,,\\
\frac{(1-\gamma)(1-\delta)}{(1+\gamma)} N_{s/(1-\gamma)} 
\leq N \leq (1+\gamma)^3 N_{s/(1+\gamma)}+ (1+\gamma) \frac{\delta}{s}\,. 
\end{gather*}
\end{lem}

Lemma \ref{lem:estCorrect} implies the following corollary, which immediately implies
the correctness of Algorithm~\ref{alg:kSparse}.

\begin{cor}
\label{cor:estCorrect}
\begin{enumerate}
\item[(a)]
If $\psi$ is $k$-supported, then, with probability at least 2/3, 
Algorithm \ref{alg:kSparse} obtains estimates $W, N$ that satisfy
$W\geq 1-\frac{\eps}{3}$ and $N\leq (1+\frac{\eps}{4})k$
\item[(b)]
If $f$ is $\eps$-far from being $k$-supported, then, 
with probability at least 2/3, 
Algorithm \ref{alg:kSparse} obtains an estimate $W:W< 1-\frac{\eps}{3}$ or
an estimate $N:N> (1+\frac{\eps}{4})k$.
\end{enumerate}
\end{cor}

We postpone the proofs of Lemma \ref{lem:estCorrect} and Corollary~\ref{cor:estCorrect} 
to the next subsection and continue with the bound on the running time now.

We call the subroutine in Step 2 of \rf(sbrtn:estimateNW) the Inner Subroutine.
It takes \onote{typo below} \bnote{Which $a$ is used in $p_a$?}
\[ 
O\left(1+ \frac{\log 1/\delta}{\gamma\sqrt{p_a}}\right) = 
O\left(\frac{\sqrt{k} \log k}{\eps}\right)
\] 
queries.  \rf(sbrtn:estimateNW) repeats the Inner Subroutine 
\[ O\left(\ell \frac{1}{\gamma} \log \ell \right) = O \left(\frac{\ell\log\ell}{\eps}\right) \] 
times, where $\ell=\log k$.\onote{can one really get multiplicative precision $1\pm \gamma$ with running time independent of the success probability of the algorithm?! We could solve NP hard question that way!} Algorithm~\ref{alg:kSparse} repeats \rf(sbrtn:estimateNW) a constant number of times. 
Therefore, the overall number of queries in Algorithm \ref{alg:kSparse} is
\[ O\left(\frac{\sqrt{k} \log^2 k \log \log k}{\eps^2}\right) .\]
The time complexity can be estimated similarly.
\pfend

\subsection{Proof of \rf(lem:estCorrect)}

We first prove a counterpart of the lemma under the assumption that \rf(sbrtn:estimateNW)
makes no error estimating the acceptance probability of the Inner Subroutine.
Let $\tW$ and $\tN$ be the output of \rf(sbrtn:estimateNW) under this assumption.
%Later we waive this assumption.

\begin{lem}
\label{lem:estCorrect1}
In notation of \rf(lem:estCorrect),
\begin{gather*}
 (1-\delta) W_{s/(1-\eps)} \leq \tilde{W} \leq W_{s/(1+\eps)} + \delta , \\
 \frac{1-\delta}{(1+\gamma)} N_{s/(1-\eps)} 
 \leq \tilde{N} \leq (1+\gamma)^2 N_{s/(1+\eps)}+ \frac{\delta}{s} .
\end{gather*}  
\end{lem}

Lemma \ref{lem:estCorrect} is implied by this lemma, as follows. 
With probability at least $1-\frac{\ell}{3\ell} = 2/3$, all $\ell$ calls of amplitude estimation in
\rf(sbrtn:estimateNW) output estimates that are within $\gamma$ fraction
of the actual values. If this happens, $(1-\gamma) W \leq \tilde{W} \leq (1+\gamma) W$ and 
$(1-\gamma) N \leq \tilde{N} \leq (1+\gamma) N$ and Lemma~\ref{lem:estCorrect}
immediately follows from Lemma~\ref{lem:estCorrect1}.

\pfstart[Proof of \rf(lem:estCorrect1)]
For $a\in[n]$, let $q_i(a)$ be the probability of 
the Inner Subroutine producing an estimate
$r \in [s_i, s_{i+1}]$, conditional on the algorithm 
sampling $a$ in the previous step.

We define the {\emph{contribution} of $a$ to $\tilde{W}$ (which we denote by $W(a)$)
as $p_a \sum_{i=0}^{\ell-1} q_i(a)$ and the {\emph{contribution} of $a$ to $\tilde{N}$ 
(which we denote by $N(a)$) as $p_a \sum_{i=0}^{\ell-1} \frac{q_i(a)}{s_i}$.
It is easy to show that $\tilde{W}=\sum_a W(a)$ and $\tilde{N}=\sum_a N(a)$. 
%(This follows by expressing each $A(p_i, p_{i+1}, \eps, \delta)$ in equations (\ref{eq:w}) and (\ref{eq:n}) as a sum over $S$ that can be sampled by the Inner Subroutine and then changing the order of summation so that we sum over $S$ first.)  

\paragraph{Lower bound on $\tilde{W}$}
Let $a$ be such that $p_a\geq s/(1-\gamma/3)$. Then, $a$ is sampled by
the Inner Subroutine with probability $p_a$ and, conditional on it 
being sampled, amplitude estimation in the Inner Subroutine gives an
estimate $\ge(1-\gamma/3) p_a \geq s$ with probability at 
least $1-\delta$. Therefore, the contribution $W(a)$ is at least $(1-\delta) p_a$.
The lower bound on $\tilde{W}$ follows by summing over all $a$.

\paragraph{Lower bound on $\tilde{N}$}
Assume $p_a \in [s_i, s_{i+1}]$. With probability at least $1-\delta$, the estimate 
for $p_a$ will be in the interval $[(1-\gamma/3) p_a, 
(1+\gamma/3) p_a]$. Thus,
\[(1+\gamma/3) p_a < (1+\gamma/3) s_{i+1} < s_{i+2}.\]
Hence, with probability at least $1-\delta$, the estimate belongs to $[s_j, s_{j+1}]$ for
$j\leq i+1$. Therefore, the contribution of 
$a$ to $\tilde{N}$ is 
%\begin{align*}
%N(a) &\geq p_a \sum_{j=0}^{i+1} \frac{q_j(a)}{s_j} \geq
%p_a \sum_{j=0}^{i+1} \frac{q_j(a)}{s_{i+1}} \\
%&\geq (1-\delta) \frac{|\widehat{f}(S)|^2}{p_{i+1}} \geq (1-\delta) \frac{p_i}{p_{i+1}}
%\geq \frac{1-\delta}{1+\gamma} \,.
%\end{align*}
\[
N(a) \geq p_a \sum_{j=0}^{i+1} \frac{q_j(a)}{s_j} \geq
p_a \sum_{j=0}^{i+1} \frac{q_j(a)}{s_{i+1}}
\geq (1-\delta) \frac{|\widehat{f}(S)|^2}{p_{i+1}} \geq (1-\delta) \frac{p_i}{p_{i+1}}
\geq \frac{1-\delta}{1+\gamma} \,.
\]

Again, the lower bound follows by summing over all $a$.

\paragraph{Upper bound on $\tilde{W}$}
Assume $a$ is such that $p_a \geq s/(1+\gamma/3)$.
Then, the contribution $W(a)\le p_a$. (This is the maximum possible value for $W(a)$, achieved if the
amplitude estimation in the Inner Subroutine always produces an estimate 
that is at least $s$.) Summing over all such $a$ gives 
$\sum_a W(a)\leq W_{s/(1+\gamma/3)}$.

If $a$ is such that $p_a < s/(1+\gamma/3)$, the probability of the
amplitude estimation in the Inner Subroutine producing an estimate 
$r\geq s$ is at most $\delta$. Therefore, $W(a) \leq \delta p_a$ and 
the sum of all such $W(a)$ is at most $\delta$.

\paragraph{ Upper bound on $\tilde{N}$}
Assume $a$ is such that $p_a\geq s/(1+\gamma/3)$.
With probability at least $1-\delta$, the estimate for $p_a$ will be in the interval 
$[(1-\gamma/3) p_a, (1+\gamma/3) p_a]$.
If $p_a \in [s_i, s_{i+1}]$, we have
\[ \skB[(1-\gamma/3) p_a, (1+\gamma/3) p_a] \subseteq [s_{i-1}, s_i] \cup [s_i, s_{i+1}] \cup [s_{i+1},
s_{i+2}] .\]
Therefore, the contribution of $S$ will be at most
\[ (1-\delta) \frac{p_a}{s_{\max\{i-1, 0\}}} + \delta \frac{p_a}{s} \]
with the first term coming from the cases when the estimate is in  
$[(1-\gamma/3) p_a, (1+\gamma/3) p_a]$ and the second term 
coming from the cases when the estimate is outside this interval.
For the denominator of the first term, we have
\[ s_{\max\{i-1, 0\}} \geq \frac{s_{i+1}}{(1+\gamma)^2} \geq  
\frac{p_a}{(1+\gamma)^2} .\]
Therefore, 
\[ N(a) \leq 
(1-\delta)(1+\gamma)^2 + \delta \frac{p_a}{s_0} 
\leq (1+\gamma)^2 + \delta \frac{p_a}{s_0} .\]
If $a$ is such that $p_a\geq s/(1+\gamma/3)$, we only get the 
second term (from the case when estimate is more than than $(1+\gamma/3) p_a$).
Summing over all $a$ gives the upper bound on $N$.
\pfend



\subsection{Proof of \rf(cor:estCorrect)}

\paragraph{Case (a)}
If $\psi$ is $k$-supported, we have $N_s\leq k$ for any $s$.
Therefore, by Lemma~\ref{lem:estCorrect}, we have
\[ N \leq (1+\gamma)^3 k + \sB[1+\gamma] \frac{\delta}{s} =
\sB[1+\frac{\eps}{6}] k + (1+\gamma) \frac{\eps}{4k} \]
which is less than $(1+\eps/4)k$, as long as $k\geq 2$.

For the bound on $W$, we observe that 
\[ W_{ s/(1-\gamma)}\geq 1- \frac{k}{1-\gamma} s = 
1 - \frac{\eps}{4(1-\gamma)}  \]
where the inequality is true because there are at most $k$ non-zero
$p_a$ that are less than $s/(1-\gamma)$. 
Combining this with the lower bound on $W$ from Lemma~\ref{lem:estCorrect}, we get
\[ W \geq (1-\gamma)(1-\delta) \left( 1 - \frac{\eps}{4(1-\gamma)} \right) 
\geq 1 - \gamma - \delta - \frac{\eps}{4(1-\gamma)} .\]
Since $\gamma \leq \eps/15$ and $\delta = \sA[\eps/(4k)]^2$,
we have $W\geq (1- \eps/3)k$, as long as $\eps$ is not too
large and $k$ is not too small.

\paragraph{Case (b)}
 Assume that $W \geq 1- \eps/3$. (Otherwise, (b) is obviously true.)
This means that 
\[ W_{s/(1+\gamma)}  > \frac{1}{1+\gamma}
\left(1-\frac{\eps}{3} - (1+\gamma) \frac{\delta}{s}\right) 
= \frac{1}{1+\gamma} \left( 1- \frac{\eps}{3} \eps - (1+\gamma)
\frac{\eps}{4k} \right) \]
\[  \geq (1-\gamma) \left( 1- \frac{\eps}{3}\eps - \sB[1+\gamma] \frac{\eps}{4k} \right)
\geq 1-  \frac{\eps}{3}\eps - (1+\gamma) \frac{\eps}{4k} -\gamma \]
which is at least $1-\eps/2$ if $k$ is large enough.

Since $\psi$ is $\eps$-far from being $k$-supported, the sum of
the $k$ largest $p_a$ is less than $1-\eps$. This means that 
the sum of $p_a$'s which have 
$p_a \geq s/(1+\gamma)$ 
but are not among the $k$ largest ones is at least 
$W_{s/(1+\gamma)} - (1-\eps) \geq \eps/2$.
We refer to such $S$ as {\emph{medium}.

Since the sum of the $k$ largest $p_a$ is less than $1-\eps$, the $(k+1)$'st 
largest $p_a$ must be less than $1/k$. 
This means that there must be at least $\eps k/2$ medium $a$ and 
we have $N_{s/(1+\gamma)} \geq (1+\eps/2) k$.
By the lower bound on $N$ from Lemma~\ref{lem:estCorrect}, this means 
\[ N \geq \frac{(1-\gamma)(1-\delta)}{(1+\gamma)} 
\left(1+\frac{\eps}{2}\right)k \geq \left(1+\frac{\eps}{4}\right)k .\]


